VK-G2T: Vision and Context Knowledge enhanced Gloss2Text

Existing sign language translation methods follow a two-stage pipeline: first converting the sign language video to a gloss sequence (i.e. Sign2Gloss) and then translating the generated gloss sequence into a spoken language sentence (i.e. Gloss2Text). While previous studies have focused on boosting the performance of the Sign2Gloss stage, we emphasize the optimization of the Gloss2Text stage. However, this task is non-trivial due to two distinct features of Gloss2Text: (1) isolated gloss input and (2) low-capacity gloss vocabulary. To address these issues, we propose a vision and context knowledge enhanced Gloss2Text model, named VK-G2T, which leverages the visual content of the sign language video to learn the properties of the target sentence and exploit the context knowledge to facilitate the adaptive translation of gloss words. Extensive experiments conducted on a Chinese benchmark validate the superiority of our model.

==> 2_related_work.tex <==
\section{Related Work}

\textbf{Sign Language Translation.} 
Existing SLT models mainly involve two stages, \ie Sign2Gloss and Gloss2Text~\cite{DBLP:conf/sitis/ArvanitisCK19,DBLP:conf/coling/YinR20,DBLP:journals/pami/KollerCNB20}. 
Previous research attention has been mostly paid to optimizing the Sign2Gloss stage~\cite{DBLP:conf/iccv/MinHC021,DBLP:conf/iccv/HaoM021}. 
Specifically, they focus on first extracting temporal and spatial features from the sign language video and then utilizing sequence modeling models~(\eg long short-term memory network~(LSTM)~\cite{DBLP:journals/neco/HochreiterS97}) to recognize the gloss sequence based on the extracted visual features. 
Despite significant progress, previous studies simply adopt the existing neural machine translation models~\cite{DBLP:journals/corr/smmtl,phonenix,DBLP:conf/naacl/CaoLLCCHL022}, such as LSTM, Transformer~\cite{DBLP:conf/nips/VaswaniSPUJGKP17},  and BART~\cite{DBLP:conf/acl/LewisLGGMLSZ20}, for the second Gloss2Text stage to derive the final spoken language translation. 


Beyond the existing studies that focus on optimizing the Sign2Gloss stage, we aim to boost the Gloss2Text performance by incorporating the visual modality of the sign language video for the target sentence property learning and exploiting the context knowledge for adaptive Gloss2Text translation. 


% \subsection{General Machine  Translation}
% \vspace{5pt}
\noindent\textbf{General Machine  Translation.} 
General machine translation, which aims to translate a source sentence into the target sentence of another language, has attracted massive research attention due to its tremendous commercial value~\cite{DBLP:journals/jair/GattK18}. 
Early studies mainly devise the algorithm based on the syntactic information and linguistically motivated rules~\cite{DBLP:conf/coling/VisweswariahNSCK10,DBLP:conf/ssst/HatakoshiNSTN14}. These methods relied heavily on hand-crafted expert knowledge and lacked flexibility when dealing with diverse languages. 
Later, with the advances of deep learning, several studies have been dedicated to exploring the capability of sequence-to-sequence neural networks towards accurate machine translation, where the common backbones are recurrent neural network (RNN)~\cite{DBLP:journals/corr/BahdanauCB14}, convolutional neural network~\cite{DBLP:conf/icml/GehringAGYD17}, and Transformer~\cite{DBLP:conf/nips/VaswaniSPUJGKP17}. 
More recently, to exploit knowledge contained in the large-scale unlabeled corpus, pretraining-based models, such as BART and DEEP~\cite{DBLP:conf/acl/0001HCN22}, have been proposed for the machine translation and achieved significant progress. 


Although these models have achieved compelling success in general translation, directly applying them to the task of Gloss2Text can only yield sub-optimal performance due to its isolated gloss input and low-capacity gloss vocabulary. 


